Global Convergence of Online Limited Memory BFGS

Global convergence of an online (stochastic) limited memory version of the Broyden-Fletcher- Goldfarb-Shanno (BFGS) quasi-Newton method for solving optimization problems with stochastic objectives that arise in large scale machine learning is established. Lower and upper bounds on the Hessian eigenvalues of the sample functions are shown to suffice to guarantee that the curvature approximation matrices have bounded determinants and traces, which, in turn, permits establishing convergence to optimal arguments with probability 1. Numerical experiments on support vector machines with synthetic data showcase reductions in convergence time relative to stochastic gradient descent algorithms as well as reductions in storage and computation relative to other online quasi-Newton methods. Experimental evaluation on a search engine advertising problem corroborates that these advantages also manifest in practical applications.

==> Convergence.tex <==
%!TEX root = root.tex
%\renewcommand \blue[1] {} \renewcommand \red[1] {}
%\newpage
\section{Convergence}\label{sec_convergence}

For the subsequent analysis it is convenient to define the instantaneous objective function associated with samples $\tbtheta=[\bbtheta_1,\ldots,\bbtheta_L]$ as
%
\begin{equation}\label{eqn_isntantaneous_dual_function}
   \hhatf(\bbw,{\tbtheta}) := \frac{1}{L}\sum_{l=1}^L f(\bbw,{\bbtheta_{l}}).
\end{equation}
% 
The definition of the instantaneous objective function $ \hhatf(\bbw,{\tbtheta})$ in association with  the fact that $F(\bbw) := \mbE_{\bbtheta}[f(\bbw,{\bbtheta})]$ implies
%
\begin{equation}\label{eqn_dual_function_as_expectation_of_isntantaneous_dual_function}
   F(\bbw) = \mbE_{\bbtheta}[\hhatf(\bbw,{\tbtheta})].
\end{equation}
%
Our goal here is to show that as time progresses the sequence of variable iterates $\bbw_t$ approaches the optimal argument $\bbw^*$. In proving this result we make the following assumptions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   A   S   S   U   M   P   T   I   O   N   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{assumption}\label{ass_intantaneous_hessian_bounds}\normalfont  The instantaneous functions $\hhatf(\bbw,{\tbtheta})$ are twice differentiable and the eigenvalues of the instantaneous Hessian $\hat{ \bbH}(\bbw,{\tbtheta} )=\nabla_{\bbw}^2\hhatf(\bbw,{\tbtheta})$ are  bounded between constants $0<\tdm$ and $\tdM<\infty$ for all random variables $\tbtheta$,
%
\begin{equation}\label{hassan}
   \tdm\bbI \ \preceq\ \hat{ \bbH}(\bbw,{\tbtheta}) \ \preceq \ \tdM \bbI.
\end{equation} \end{assumption}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   A   S   S   U   M   P   T   I   O   N   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{assumption}\normalfont\label{ass_bounded_stochastic_gradient_norm} The second moment of the norm of the stochastic gradient is bounded for all $\bbw$. i.e., there exists a constant $S^2$ such that for all variables $\bbw$ it holds
%
\begin{equation}\label{ekhtelaf}
   \mbE_{\bbtheta} \big{[} \| \hbs(\bbw_{t},\tbtheta_{t})\|^{2} \big{]} \leq S^{2}, 
\end{equation} \end{assumption}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%   A   S   S   U   M   P   T   I   O   N   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%\begin{assumption}\normalfont\label{ass_delta_less_m} The regularization constant $\delta$ is smaller than the smallest Hessian eigenvalue $\tdm$, i.e., $\delta<\tdm$.
%\end{assumption}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
As a consequence of Assumption \ref{ass_intantaneous_hessian_bounds} similar eigenvalue bounds hold for the (average) function $F(\bbw)$. Indeed, it follows from the linearity of the expectation operator and the expression in \eqref{eqn_dual_function_as_expectation_of_isntantaneous_dual_function} that the Hessian is $\nabla_{\bbw}^{2}F(\bbw)= \bbH(\bbw)=\mbE_{\bbtheta}[\hat{\bbH}(\bbw,{\tbtheta})]$. Combining this observation with the bounds in \eqref{hassan} it follows that there are constants $m\geq\tdm$ and $M\leq\tdM$ such that
%
\begin{equation}\label{bbb}
   \tdm\bbI \ \preceq\ m\bbI\ \preceq\ \bbH(\bbw) \ \preceq  M\bbI \ \preceq \ \tdM\bbI.
\end{equation} 
%
The bounds in \eqref{bbb} are customary in convergence proofs of descent methods. For the results here the stronger condition spelled in Assumption \ref{ass_intantaneous_hessian_bounds} is needed. The restriction imposed by Assumption \ref{ass_bounded_stochastic_gradient_norm} is typical of stochastic descent algorithms, its intent being to limit the random variation of stochastic gradients. Assumption \ref{ass_delta_less_m} is necessary to guarantee that the inner product $\tbr_{t}^{T}\bbv_{t}=(\bbr_t-\delta\bbv_t)^T\bbv_t>0$ [cf. Proposition \ref{flen}] is positive as we show in the following lemma.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   L   E   M   M   A   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{lemma}\label{lecce}
Consider the modified stochastic gradient variation $\tbr_{t}$ defined in \eqref{chris2} and the variable variation $\bbv_{t}$ defined in \eqref{ball}. Let Assumption \ref{ass_intantaneous_hessian_bounds} hold and recall the lower bound $\tdm$ on the smallest eigenvalue of the instantaneous Hessians. Then, for all constants $\delta < \tdm$ it holds
%
\begin{equation}\label{claim233}
   \tbr_{t}^{T}\bbv_{t} \ =\ (\hbr_{t}-\delta \bbv_{t})^T\bbv_{t}\ \geq (\tdm-\delta) \|\bbv_{t}\|^{2} \ >\ 0.
\end{equation}\end{lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   P   R   O   O   F   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{myproof} 
As per \eqref{hassan} in Assumption 1 the eigenvalues of the instantaneous Hessian $\hat{ \bbH}(\bbw,{\tbtheta})$ are bounded by $\tdm$ and $\tdM$. Thus, for any given vector $\bbz$ it holds
%
\begin{equation}\label{liverpool}
\tdm \|\bbz\|^{2} \leq \bbz^{T} \hat{ \bbH}(\bbw,{\tbtheta}) \bbz \leq \tdM \|\bbz\|^{2}.
\end{equation}
%
For given $\bbw_{t}$ and $\bbw_{t+1}$ define the mean instantaneous Hessian $\hbG_{t}$ as the average Hessian value along the segment $[\bbw_{t},\bbw_{t+1}]$
%
\begin{equation}\label{average}
\hbG_{t}= \int_{0}^{1}  \hat{ \bbH} \left( \bbw_{t}+\tau(\bbw_{t+1}-\bbw_{t}),{\tbtheta_{t}}\right) d\tau.
\end{equation}
%
Consider now the instantaneous gradient $\hbs( \bbw_{t}+\tau(\bbw_{t+1}-\bbw_{t}),\tbtheta_{t})$ evaluated at $\bbw_{t}+\tau(\bbw_{t+1}-\bbw_{t})$ and observe that its derivative with respect to $\tau$ is $\partial\hbs\big( \bbw_{t}+\tau(\bbw_{t+1}-\bbw_{t}),\tbtheta_{t}\big)/\partial \tau = \hbH(\bbw_{t}+\tau( \bbw_{t+1} - \bbw_{t}),{\tbtheta_{t}})  (\bbw_{t+1} - \bbw_{t})$. It then follows from the fundamental theorem of calculus that 
%
\begin{align}\label{lazio}
   \int_{0}^{1}\!\hbH ( \bbw_{t}+\tau(\bbw_{t+1}-\bbw_{t}),{\tbtheta_{t}} )  
                        (\bbw_{t+1} - \bbw_{t})\ d\tau  
      = \nonumber \\
       \hbs(\bbw_{t+1},\tbtheta_{t}) - \hbs(\bbw_{t},\tbtheta_{t}) .
\end{align}
%
Using the definitions of the mean instantaneous Hessian $\hbG_{t}$ in \eqref{average} as well as the definitions of the stochastic gradient variations $\hbr_{t}$ and variable variations $\bbv_{t}$ in \eqref{chris} and \eqref{ball} we can rewrite \eqref{lazio} as
%
\begin{equation}\label{mancity}
 \hbG_{t} \bbv_{t} = \hbr_{t}.
\end{equation}
%
Invoking \eqref{liverpool} for the integrand in \eqref{average}, i.e., for $\hat{ \bbH}(\bbw,{\tbtheta}) = \hat{ \bbH}\big{(}\bbw_{t}+\tau(\bbw_{t+1}-\bbw_{t}),{\tbtheta} \big{)}$, it follows that for all vectors $\bbz$ the mean instantaneous Hessian $\hbG_{t}$ satisfies
%
\begin{equation}\label{arsenal}
   \tdm \|\bbz\|^{2} \leq \bbz^{T} \hbG_{t} \bbz \leq \tdM \|\bbz\|^{2}.
\end{equation}
%
{The claim in \eqref{claim233} follows from \eqref{mancity} and \eqref{arsenal}.} Indeed, consider the ratio of inner products $\hbr_{t}^{T}\bbv_{t}/\bbv_{t}^{T}\bbv_{t}$ and use \eqref{mancity} and the first inequality in \eqref{arsenal} to write
 %
\begin{equation}\label{jose}
   \frac{\hbr_{t}^{T}\bbv_{t}}{\bbv_{t}^{T}\bbv_{t}}
       = \frac{{\bbv_{t}^{T} \hbG_{t} \bbv_{t} }}{\bbv_{t}^{T} \bbv_{t}} \geq \tdm.
\end{equation}
%
%Since the first inequality in \eqref{arsenal} implies that the mean instantaneous Hessian matrix $\hbG_{t}$ is positive definite its square root $\hbG_{t}^{1/2}$ is well defined. We can then define the vector $\bbz_{t}:= \hbG_{t}^{{1}\over{2}} \bbmu_{t}$ in order to rewrite \eqref{jose} as
%%
%\begin{equation}\label{jose2}
%    \frac{\hbr_{t}^{T}\hbr_{t}}{\hbr_{t}^{T}\bbmu_{t}} 
%        = \frac{\bbz_{t}^{T} \hbG_{t} \bbz_{t}}{\bbz_{t}^{T}\bbz_{t}} \leq \tdM,
%\end{equation}
%%
%where the inequality follows from \eqref{arsenal} with $\bbz=\bbz_t$. 
Consider now the inner product $\tbr_{t}^{T}\bbv_{t} \ =\ (\hbr_{t}-\delta \bbv_{t})^T\bbv_{t}$ in \eqref{claim233} and use the bound in \eqref{jose} to write
%
\begin{align}\label{bound_for_norm_r}
   \tbr_{t}^{T}\bbv_{t}
      \ =   \  \hbr_{t}^{T}\bbv_{t} - \delta  \bbv_{t}^{T}\bbv_{t}
      \ \geq\  {{\tdm}}\bbv_{t}^{T}\bbv_{t} - \delta  \bbv_{t}^{T}\bbv_{t}
\end{align}
% 
Since we are selecting $\delta < \tdm$ by hypothesis it follows that \eqref{claim233} is true for all times $t$. \end{myproof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Initializing the curvature approximation matrix $\hbB_0\succ\delta\bbI$, which implies $\hbB_0^{-1}\succ\bbzero$, and setting $\delta < \tdm$ it follows from Lemma \ref{lecce} that the hypotheses of Proposition \ref{flen} are satisfied for $t=0$. Hence, the matrix $\hbB_1$ computed from \eqref{akbar} is the solution of the semidefinite program in \eqref{jadid} and, more to the point, satisfies $\hbB_1\succ\delta\bbI$, which in turn implies  $\hbB_1^{-1}\succ\bbzero$. Proceeding recursively we can conclude that $\hbB_{t}\succ\delta\bbI\succ\bbzero$ for all times $t\geq0$. Equivalently, this implies that all the eigenvalues of $\hbB_t^{-1}$ are between $0$ and $1/\delta$ and that, as a consequence, the matrix $\hbB_t^{-1}+\Gamma \bbI$ is such that
%
\begin{equation}\label{eqn_eigenvalue_critical_bounds}
   \Gamma \bbI
      \ \preceq\ \hbB_t^{-1}+\Gamma \bbI  
      \ \preceq\ \left(\Gamma+\frac{1}{\delta}\right) \bbI.
\end{equation} 
%
Having matrices $\hbB_t^{-1}+\Gamma \bbI$ that are strictly positive definite with eigenvalues uniformly upper bounded by $\Gamma+(1/\delta)$ leads to the conclusion that if $\hbs(\bbw_{t},\tbtheta_{t})$ is a descent direction, the same holds true of $(\hbB_t^{-1}+\Gamma \bbI)\ \! \hbs(\bbw_{t},\tbtheta_{t})$. The stochastic gradient $\hbs(\bbw_{t},\tbtheta_{t})$ is not a descent direction in general, but we know that this is true for its conditional expectation $\mbE[\hbs(\bbw_{t},\tbtheta_{t}) \given \bbw_{t}] = \nabla_{\bbw} F(\bbw_{t})$. Therefore, we conclude that $(\hbB_t^{-1}+\Gamma \bbI)\ \! \hbs(\bbw_{t},\tbtheta_{t})$ is an average descent direction because $\mbE[(\hbB_t^{-1}+\Gamma \bbI)\ \!\hbs(\bbw_{t},\tbtheta_{t}) \given \bbw_{t}] = (\hbB_t^{-1}+\Gamma \bbI)\ \! \nabla_{\bbw} F(\bbw_{t})$. Stochastic optimization algorithms whose displacements $\bbw_{t+1}-\bbw_t$ are descent directions on average are expected to approach optimal arguments in a sense that we specify formally in the following lemma.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   L  E  M  M  A  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{lemma}\label{helpful}
Consider the RES algorithm as defined by \eqref{eqn_sbfgs_dual_iteration}-\eqref{akbar}. If assumptions \ref{ass_intantaneous_hessian_bounds}, \ref{ass_bounded_stochastic_gradient_norm} and \ref{ass_delta_less_m} hold true, the sequence of average function $F(\bbw_{t})$ satisfies
%
\begin{equation}\label{pedarsag}
    \E{F(\bbw_{t+1})\given \bbw_{t}}  
         \leq F(\bbw_{t})
          -  \epsilon_{t} \Gamma \| \nabla F(\bbw_{t})\|^{2} 
          + K \epsilon_{t}^{2}
\end{equation}
%
where the constant $K:={MS^{2}} ({1/\delta}+\Gamma)^{2} /2$.

\end{lemma}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   P   R   O   O   F   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{myproof} 
As it follows from Assumption 1 the eigenvalues of the Hessian $\bbH(\bbw_{t})=\mbE_{\tbtheta}[\hbH(\bbw_{t},\tbtheta_{t})] = \nabla_{\bbw}^{2} F(\bbw_{t})$ are bounded between $0<m$ and $M<\infty$ as stated in \eqref{bbb}. Taking a Taylor's expansion of the dual function $F(\bbw)$ around $\bbw=\bbw_{t}$ and using the upper bound in the Hessian eigenvalues we can write
%
\begin{equation}\label{taylor_upper_bound}
   F(\bbw_{t+1}) \leq F(\bbw_{t}) +\nabla F(\bbw_{t})^{T}\!(\bbw_{t+1}-\bbw_{t})   
   + {{M}\over{2}}\|{\bbw_{t+1}-\bbw_{t}}\|^{2}
\end{equation}
%
From the definition of the RES update in \eqref{eqn_sbfgs_dual_iteration} we can write the difference of two consecutive variables   $\bbw_{t+1}-\bbw_{t} $ as $ -\epsilon_{t}(\hbB_{t}^{-1}+\Gamma \bbI )\ \hbs(\bbw_{t},\tbtheta_{t})$. Making this substitution in \eqref{taylor_upper_bound}, taking expectation with $\bbw_{t}$ given in both sides of the resulting inequality, and observing the fact that when $\bbw_{t}$ is given the Hessian approximation $\hbB_{t}^{-1}$ is deterministic we can write
%
\begin{align}\label{pedar_sag}
  &  \E{F(\bbw_{t+1})\given \bbw_{t}}  \leq\  F(\bbw_{t})  \\ & \qquad\qquad\qquad 
          - \epsilon_{t}\nabla F(\bbw_{t})^{T}(\hbB_{t}^{-1}+\Gamma \bbI )
                 \E{\hbs(\bbw_{t},\tbtheta_{t})\given\bbw_{t}} \nonumber\\&\qquad\qquad\qquad
          + \frac{\epsilon^{2}M}{2} \ \!
              \E{\left\|(\hbB_{t}^{-1}+\Gamma \bbI )\hbs(\bbw_{t},\tbtheta_{t})\right\|^{2} 
                    \given \bbw_{t}}. \nonumber
\end{align}
%
We proceed to bound the third term in the right hand side of \eqref{pedar_sag}. Start by observing that the 2-norm of a product is not larger than the product of the 2-norms and that, as noted above, with $\bbw_{t}$ given the matrix $\hbB_{t}^{-1}$ is also given to write 
%
\begin{align}\label{pedar_salavati}
    &\E{\left\| \left(\hbB_{t}^{-1}+\Gamma \bbI\right)\hbs(\bbw_{t},\tbtheta_{t})\right\|^{2} 
            \given \bbw_{t}}  \nonumber\\  &\hspace{24mm} 
     \leq  \left\|\hbB_{t}^{-1}+\Gamma \bbI \right\|^{2}   
           \E{\left\|  \hbs(\bbw_{t},\tbtheta_{t})\right\|^{2} \given \bbw_{t}}.
\end{align}
%
Notice that, as stated in \eqref{eqn_eigenvalue_critical_bounds}, $\Gamma + 1/\delta$ is an upper bound for the eigenvalues of $\hbB_{t}^{-1}+\Gamma \bbI$. Further observe that the second moment of the norm of the stochastic gradient is bounded by $  \E{\| \hbs(\bbw_{t},\tbtheta_{t})\|^{2} \given \bbw_{t}} \leq S^{2}$, as stated in Assumption 2. These two upper bounds  substituted in \eqref{pedar_salavati} yield
%
\begin{equation}\label{dash_akol}
    \E{\left\| \left(\hbB_{t}^{-1}+\Gamma \bbI\right)\hbs(\bbw_{t},\tbtheta_{t})\right\|^{2} 
           \given \bbw_{t}}\leq S^2(1/\delta+\Gamma)^{2}.
\end{equation}
%
Substituting the upper bound in \eqref{dash_akol} for the third term of \eqref{pedar_sag} and further using the fact that $ \E{\hbs(\bbw_{t},\tbtheta_{t})\given\bbw_{t}}=\nabla F(\bbw_{t})$ in the second term leads to
%
\begin{align}\label{lavashak}
    \E{F(\bbw_{t+1})\given \bbw_{t}}  
          \leq & F(\bbw_{t})   -  \epsilon_{t} \nabla F(\bbw_{t})^{T}\! \left(\hbB_{t}^{-1}+\Gamma \bbI\right)       \! \nabla F(\bbw_{t}) 
        \nonumber \\ &
          \quad  
          +\frac{\epsilon_{t}^{2}MS^{2}}{{2}} (1/\delta+\Gamma)^{2}  .
\end{align}
%
We now find a lower bound for the second term in the right hand side of \eqref{lavashak}. Since the Hessian approximation matrices $\hbB_{t}$ are positive definite their inverses $\hbB_{t}^{-1}$ are positive semidefinite. In turn, this implies that all the eigenvalues of $\hbB_{t}^{-1}+ \Gamma \bbI$ are not smaller than $\Gamma$ since $\Gamma \bbI$ increases all the eigenvalues of $\hbB_{t}^{-1}$ by $\Gamma$. This lower bound for the eigenvalues of $\hbB_{t}^{-1}+ \Gamma \bbI$ implies that
%
\begin{equation}\label{inner_product_lower_bound}
   \nabla F(\bbw_{t})^{T} \left(\hbB_{t}^{-1}+\Gamma \bbI\right)\nabla F(\bbw_{t}) 
       \geq \Gamma \|\nabla F(\bbw_{t}) \|^{2} 
\end{equation}  
%
Substituting the lower bound in \eqref{inner_product_lower_bound} for the corresponding summand in \eqref{lavashak} and further noting the definition of $K:={MS^{2}} ({1/\delta}+\Gamma)^{2} /2$  in the statement of the lemma, the result in \eqref{taylor_upper_bound} follows.

\end{myproof}

Setting aside the term $K\eps_t^2$ for the sake of argument \eqref{pedarsag} defines a supermartingale relationship for the sequence of average functions $F(\bbw_{t})$. This implies that the sequence $\eps_t\Gamma\ \| \nabla F(\bbw_{t})\|^{2}$ is almost surely summable which, given that the step sizes $\eps_t$ are nonsummable as per \eqref{stepsize_condition}, further implies that the limit infimum $\liminf_{t\to\infty}\|\nabla F(\bbw_{t})\|$ of the gradient norm $\|\nabla F(\bbw_{t})\|$ is almost surely null. This latter observation is equivalent to having $\liminf_{t\to\infty}\| \bbw_{t}-\bbw^{*} \|^{2} =0$ with probability 1 over realizations of the random samples $\{\tbtheta_t\}_{t=0}^\infty$. The term $K\eps_t^2$ is a relatively minor nuisance that can be taken care with a technical argument that we present in the proof of the following theorem.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   T   H   E   O   R   E   M   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{thm}\label{convg}
Consider the RES algorithm as defined by \eqref{eqn_sbfgs_dual_iteration}-\eqref{akbar}. If assumptions \ref{ass_intantaneous_hessian_bounds}, \ref{ass_bounded_stochastic_gradient_norm} and \ref{ass_delta_less_m} hold true and the sequence of stepsizes satisfies \eqref{stepsize_condition}, the limit infimum of the squared Euclidean distance to optimality $\| \bbw_{t}-\bbw^{*} \|^{2}$ satisfies
%
\begin{equation}\label{eqn_convg}
   \liminf_{t \to \infty }\| \bbw_{t}-\bbw^{*} \|^{2} = 0 \qquad \text{a.s.}
\end{equation} 
over realizations of the random samples $\{\tbtheta_t\}_{t=0}^\infty$.\end{thm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   P   R   O   O   F   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{myproof} 
The proof uses the relationship in the statement \eqref{pedarsag} of Lemma \ref{helpful} to build a supermartingale sequence. For that purpose define the stochastic process $\gamma_t$ with values 
%
\begin{equation}\label{alp}
   \gamma_t := F(\bbw_{t})+ K \sum_{u=t}^{\infty}  {{\epsilon_{u}^{2}}}.
\end{equation}
%
Observe that $\gamma_t$ is well defined because the $\sum_{u=t}^{\infty}  {{\epsilon_{u}^{2}}}<\sum_{u=0}^{\infty}  {{\epsilon_{u}^{2}}}<\infty$ is summable. Further define the sequence $\beta_t$ with values
%
\begin{equation}\label{beta}
   \beta_t :=\ \epsilon_{t}\ \Gamma\ \| \nabla F(\bbw_{t})\|^{2} .
\end{equation}
%
Let now $\ccalF_t$ be a sigma-algebra measuring $\gamma_t$, $\beta_t$, and $\bbw_t$. The conditional expectation of $\gamma_{t+1}$ given $\ccalF_t$ can be written as
%
\begin{equation}\label{eqn_theo_convg_pf_30}
   \E{\gamma_{t+1} \given \ccalF_t} 
       =  \E{F(\bbw_{t}) \given \ccalF_t}
             + K \sum_{u=t}^{\infty}  {{\epsilon_{u}^{2}}},
\end{equation}
%
because the term $K \sum_{u=t}^{\infty}  {{\epsilon_{u}^{2}}}$ is just a deterministic constant. Substituting \eqref{pedarsag} of Lemma \ref{helpful} into \eqref{eqn_theo_convg_pf_30} and using the definitions of $\gamma_t$ in \eqref{alp} and $\beta_t$ in \eqref{beta} yields
%
\begin{equation}\label{martin}
   \E{\gamma_{t+1} \given \gamma_t} \ \leq\ \gamma_t - \beta_t
\end{equation}
%
Since the sequences $\gamma_t$ and $\beta_t$ are nonnegative it follows from \eqref{martin} that they satisfy the conditions of the supermartingale convergence theorem -- {see e.g. theorem E$7.4$ \cite{Solo}} . Therefore, we conclude that: (i) The sequence $\gamma_t$ converges almost surely. (ii) The sum $\sum_{t=0}^{\infty}\beta_t < \infty$ is almost surely finite. Using the explicit form of $\beta_t$ in \eqref{beta} we have that $\sum_{t=0}^{\infty}\beta_t < \infty$ is equivalent to
%
\begin{equation}\label{psg}
   \sum_{t=0}^{\infty} \epsilon_{t}\Gamma\| \nabla F(\bbw_{t})\|^{2} < \infty, 
       \qquad\text{a.s.}
\end{equation}
%
Since the sequence of stepsizes is nonsummable for \eqref{psg} to be true we need to have a vanishing subsequence embedded in $\| \nabla F(\bbw_{t})\|^{2}$. By definition, this miles that the limit infimum of the sequence $\| \nabla F(\bbw_{t})\|^{2}$ is null,
%
\begin{equation}\label{pppp}
   \liminf_{t \to \infty}   \| \nabla F(\bbw_{t})\|^{2}  =  0,  \qquad\text{a.s.}
\end{equation}
%
To transform the gradient bound in \eqref{pppp} into a bound pertaining to the squared distance to optimality  $\| \bbw_{t} -\bbw^{*} \|^2$ simply observe that the lower bound $m$ on the eigenvalues of $\textbf{H}(\bbw_{t})$ applied to a Taylor's expansion around the optimal argument $\bbw^*$ implies that
%
\begin{equation}\label{lower_bound_taylor_expansion}
F(\bbw^*)\ \geq\ F(\bbw_{t})+  \nabla F(\bbw_{t})^{T} (\bbw^*-\bbw_{t}) 
		+\ \frac{m}{2} \|\bbw^*-\bbw_{t}\|^2 .
\end{equation}
%
Observe now that since $\bbw^*$ is the minimizing argument of $F(\bbw)$ we must have  $F(\bbw^*) -\ F(\bbw_{t}) \leq 0$ for all $\bbw$. Using this fact and reordering terms we simplify \eqref{lower_bound_taylor_expansion} to
%
\begin{equation}\label{eqn_theo_convg_pf_80}
 \frac{m}{2}\  \|\bbw^*-\bbw_{t}\|^2\  \leq\ \nabla F(\bbw_{t})^{T} (\bbw_t-\bbw^*) .
\end{equation}   
%
Further observe that the Cauchy-Schwarz inequality implies that $\nabla F(\bbw_{t})^{T} (\bbw_{t} - \bbw^*)\leq\|\nabla F(\bbw_{t})\|\|\bbw_{t}-\bbw^{*}\|$. Substitution of this bound in \eqref{eqn_theo_convg_pf_80} and simplification of a $\|\bbw^*-\bbw_{t}\|$ factor yields
%
\begin{equation}\label{qqqq}
   \frac{m}{2}\| \bbw_{t} -\bbw^{*} \|\  \leq\   \|\nabla F(\bbw_{t})\|.
\end{equation}
%
Since the limit infimum of $\|\nabla F(\bbw_{t})\|$ is null as stated in \eqref{pppp} the result in \eqref{eqn_convg} follows from considering the bound in \eqref{qqqq} in the limit as the iteration index $t\to\infty$. 

\end{myproof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
{Theorem \ref{convg} establishes convergence of the RES algorithm summarized in Algorithm \ref{algo_stochastic_bfgs}. In the proof of the prerequisite Lemma \ref{helpful} the lower bound in the eigenvalues of $\hbB_t$ enforced by the regularization in \eqref{akbar} plays a fundamental role. Roughly speaking, the lower bound in the eigenvalues of $\hbB_t$ results in an upper bound on the eigenvalues of $\hbB_t^{-1}$ which limits the effect of random variations on the stochastic gradient $\hbs(\bbw_{t},\tbtheta_{t})$. If this regularization is not implemented, i.e., if we keep $\delta=0$, we may observe catastrophic amplification of random variations of the stochastic gradient. This effect is indeed observed in the numerical experiments in Section \ref{sec:simulations}. The addition of the identity matrix bias $\Gamma\bbI$ in \eqref{eqn_sbfgs_dual_iteration} is instrumental in the proof of Theorem \ref{convg} proper. This bias limits the effects of randomness in the curvature estimate $\hbB_t$. If random variations in the curvature estimate $\hbB_t$ result in a matrix $\hbB_t^{-1}$ with small eigenvalues the term $\Gamma\bbI$ dominates and \eqref{eqn_sbfgs_dual_iteration} reduces to (regular) SGD. This ensures continued progress towards the optimal argument $\bbw^*$.} 
%\blue{After proving a theorem you comment on things that are interesting. I value that you tried doing this, but you ended up commenting on something rather trivial. Try thinking harder. These comments are very important.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> Simulations.tex <==
%!TEX root = root.tex
\section{Numerical analysis}
\label{sec:simulations}

 
We compare convergence times of RES and SGD in problems with small and large condition numbers. We use a stochastic quadratic objective function as a test case. In particular, consider a positive definite diagonal matrix $\bbA \in \mbS_{n}^{++}$, a vector $\bbb \in \mbR^{n}$, a random vector $\bbtheta\in\reals^n$, and diagonal matrix $\diag(\bbtheta)$ defined by $\bbtheta$. The function $F(\bbw)$ in \eqref{optimization_problem} is defined as
% 
\begin{align}\label{example_problem}
  F(\bbw)  :=&\ \mbE_{\theta}\left[ f(\bbw,{\theta})\right]  \nonumber \\ 
           :=&\ \mbE_{\theta} \left[\frac{1}{2}
               \bbw^{T}\Big(\bbA+\bbA\diag(\bbtheta)\Big)\bbw+\bbb^{T}\bbw\right].
\end{align}
%
In \eqref{example_problem}, the random vector $\bbtheta$ is chosen uniformly at random from the $n$ dimensional box $\Theta=[-\theta_0,\theta_0]^n$ for some given constant $\theta_0<1$. The linear term $\bbb^{T}\bbw$ is added so that the instantaneous functions $ f(\bbw,{\theta})$ have different minima  which are (almost surely) different from the minimum of the average function $F(\bbw)$. The quadratic term is chosen so that the condition number of $F(\bbw)$ is the condition number of $\bbA$. Indeed, just observe that since $\mbE_{\theta}[\bbtheta]=\bbzero$, the average function in \eqref{example_problem} can be written as $F(\bbw)=(1/2)\bbw^{T}\bbA\bbw+\bbb^{T}\bbw$. The parameter $\theta_0$ controls the variability of the instantaneous functions $f(\bbw,{\theta})$. For small $\theta_0\approx0$ instantaneous functions are close to each other and to the average function. For large $\theta_0\approx1$ instantaneous functions vary over a large range. Further note that we can write the optimum argument as $\bbw^*= \bbA^{-1}\bbb$ for comparison against iterates $\bbw_t$.

For a given $\rho$ we study the convergence metric
% 
\begin{align}\label{eqn_empirical_convergence_time}
   \tau := L \min_t \left\{ t : \frac{\|\bbw_t-\bbw^*\|}{\|\bbw^*\|} \leq \rho\right\},
\end{align}
%
which represents the time needed to achieve a given relative distance to optimality $\|\bbw_t-\bbw^*\|/\|\bbw^*\|\leq\rho$ as measured in terms of the number $Lt$ of stochastic functions that are processed to achieve such accuracy.

%\red{The regularization parameters $\delta$ and $\Gamma$ do not have a critical role in the speed of convergence for regularized stochastic BFGS. They avoid catastrophic behavior of stochastic amplification of random variable in stochastic BFGS. As we discussed in Lemma $2$ the regularization parameter $\delta$ should be less than $ \tdm$, where $\tdm$ is the minimum eigenvalue of the objective function Hessian where in this example $\tdm=10^{-\xi}$. In order to make sure that we always satisfies $\delta \leq \tdm$, we set  $\delta=10^{-3}$. Further the minimum progress parameter in \eqref{eqn_sbfgs_dual_iteration} to $\Gamma=10^{-4}$.} \blue{You have already talked about these parameters and their role. Here, you just give their values. Remove this paragraph.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth,height=0.490\linewidth]{illustration2.eps}
\caption{ Convergence of SGD and RES for the function in \eqref{example_problem}. Relative distance to optimality $\|\bbw_t-\bbw^*\|/\|\bbw^*\|$ shown with respect to the number $Lt$ of stochastic functions processed. For RES the number of iterations required to achieve a certain accuracy is smaller than the corresponding number for SGD. {See text for parameters values.} }
\label{fig:3}
\end{figure}
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsection{Effect of problem's condition number}\label{sec_numerical_analysis_condition_number}

To study the effect of the problem's condition number we generate instances of \eqref{example_problem} by choosing $\bbb$ uniformly at random from the box $[0,1]^n$ and the matrix $\bbA$ as diagonal with elements $a_{ii}$ uniformly drawn from the discrete set $\{1, 10^{-1},\ldots, 10^{-\xi}\}$. This choice of $\bbA$ yields problems with condition number $10^\xi$. 

Representative runs of RES and SGD for $n=50$, $\theta_0=0.5$, and $\xi=2$ are shown in Fig. \ref{fig:3}. For the RES run the stochastic gradients $\hbs(\bbw,\tbtheta)$ in \eqref{stochastic_gradient} are computed as an average of $L=5$ realizations, the regularization parameter in \eqref{jadid} is set to $\delta=10^{-3}$, and the minimum progress parameter in \eqref{eqn_sbfgs_dual_iteration} to $\Gamma=10^{-4}$. For SGD we use $L=1$ in \eqref{stochastic_gradient}. In both cases the step size sequence is of the form $\epsilon_{t}=\epsilon_{0}T_{0}/ (T_{0}+t)$ with  $\epsilon_{0} =10^{-1}$ and $T_{0}=10^3$. Since we are using different value of $L$ for SGD and RES we plot the relative distance to optimality $\|\bbw_t-\bbw^*\|/\|\bbw^*\|$ against the number $Lt$ of functions processed up until iteration $t$.

As expected for a problem with a large condition number RES is much faster than SGD. After $t=1,200$ the distance to optimality for the SGD iterate is {$\|\bbw_t-\bbw^*\|/\|\bbw^*\|=3.8\times10^{-2}$}. Comparable accuracy $\|\bbw_t-\bbw^*\|/\|\bbw^*\|=3.8\times10^{-2}$ for RES is achieved after $t=38$ iterations. Since we are using $L=5$ for RES this corresponds to $Lt=190$ random function evaluations. Conversely, upon processing  $Lt=1,200$ random functions -- which corresponds to $t=240$ iterations -- RES achieves accuracy $\|\bbw_t-\bbw^*\|/\|\bbw^*\|=6.6\times10^{-3}$. This relative performance difference can be made arbitrarily large by modifying the condition number of $\bbA$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth,height=0.490\linewidth]{cn_10_2.eps}
\caption{ Convergence of SGD and RES for well conditioned problems. Empirical distributions of the number $\tau=Lt$ of stochastic functions that are processed to achieve relative precision $\|\bbw_t-\bbw^*\|/\|\bbw^*\|\leq10^{-2}$ are shown. Histogram is across {$J=1,000$} realizations of functions as in \eqref{example_problem} with condition number $10^\xi=1$. Convergence for RES is better than SGD but the number of iterations required for convergence is of the same order of magnitude. See text for parameters values.
%\red{$\epsilon_0 =0.5$}
}
\label{fig:1}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth,height=0.490\linewidth]{cn_100_2.eps}
 \caption{ Convergence of SGD and RES for ill conditioned problems. Empirical distributions of the number $\tau=Lt$ of stochastic functions that are processed to achieve relative precision $\|\bbw_t-\bbw^*\|/\|\bbw^*\|\leq10^{-2}$ are shown. Histogram is across {$J=1,000$} realizations of functions as in \eqref{example_problem} with condition number $10^\xi=10^2$. RES reduces the convergence time of SGD by an order of magnitude. See text for parameters values.
 %\red{$\epsilon_0 =0.1$}
 }
\label{fig:2}
\end{figure}

A more comprehensive analysis of the relative advantages of RES appears in figs. \ref{fig:1} and \ref{fig:2}. We keep the same parameters used to generate Fig. \ref{fig:3} except that we use $\xi=0$ for Fig. \ref{fig:1} and $\xi=2$ for Fig. \ref{fig:2}. This yields a family of well-condition functions with condition number $10^\xi=1$ and a family of ill-conditioned functions with condition number  $10^\xi=10^2$. In both figures we consider $\rho=10^{-2}$ and study the convergence times $\tau$ and $\tau'$ of RES and SGD, respectively [cf. \eqref{eqn_empirical_convergence_time}]. Resulting empirical distributions of $\tau$ and $\tau'$ across {$J=1,000$ instances of the functions $F(\bbw)$ in \eqref{example_problem}} are reported in figs. \ref{fig:1} and \ref{fig:2} for the well conditioned and ill conditioned families, respectively. For the well conditioned family RES reduces the number of functions processed from an average of {$\bar\tau'=601$} in the case of SGD to an average of {$\bar\tau=144$}. This nondramatic improvement becomes more significant for the ill conditioned family where the reduction is from an average of {$\bar\tau'=7.2 \times10^3$} for SGD to an average of {$\bar\tau=3.2 \times10^2$} for RES. The spread in convergence times is also smaller for RES.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth,height=0.490\linewidth]{L_effect.eps}
\caption{ Convergence of RES for different sample sizes in the computation of stochastic gradients. Empirical distributions of the number $\tau=Lt$ of stochastic functions that are processed to achieve relative precision $\|\bbw_t-\bbw^*\|/\|\bbw^*\|\leq10^{-2}$ are shown when we use $L=1$, $L=2$, $L=5$, $L=10$, and $L=20$ in the evaluation of the stochastic gradients $\hbs(\bbw,\tbtheta)$ in \eqref{stochastic_gradient}. The average convergence time decreases as we go from small to moderate values of $L$ and starts increasing as we go from moderate to large values of $L$. The variance of convergence times decreases monotonically with increasing $L$. See text for parameters values.}
\label{fig:SSE}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsection{Choice of stochastic gradient average}
%
%\blue{WARNING: THE CASE $L=5$ HERE SHOULD COINCIDE WITH FIG. \ref{fig:2} BECAUSE THE PARAMETERS ARE THE SAME. BUT THEY DON'T. I KNOW THE DIFFERENCE IS MINIMAL, BUT TO AVOID STUPID QUESTIONS FROM REVIEWERS WE NEED TO HAVE THE SAME DATASET IN BOTH FIGURES.}

%\blue{Remember: First you explain what to do, then you dwell on consequences. Motives are irrelevant. See further comments.} \red{One of the important parameter in regularized stochastic BFGS is the sample-size $L$. Choosing a small sample-size give us a very noisy stochastic gradient, while a large sample-size increases the number of data points that the algorithm needs for convergence.} \blue {This is a motive. Motives are not relevant. You just want to say that you are studying the effect of $L$. Period.} \red{A run of regularized stochastic BFGS for different choices of sample-size is shown in Figure \ref{fig:SSE} when $\delta =10^{-3}$, $\xi=2$, $\epsilon_0=0.1$, $\tau=10^3$ and $n=50$.} \blue{This is what you do. The explanation needs to be expanded.} \red{In the case that $L=1$, most of the time the algorithm needs more than $10^3$ data points to achieve accuracy of $\|\bbw_t-\bbw^*\|/\|\bbw^*\| \leq10^{-2}$. For $L=2$ the variance of necessary number of data points for convergence is large in comparison with the case that $L=5$. The large choices of sample-size e.g. $L=10$ and $L=20$, give us a smaller variance but the average number of data points needed for convergence is more than the average of $L=5$.} \blue{A description of your consequences. Good, except that you have other interesting observations. You need to learn how to stare at data.} \red{Comparing these 5 plots imply that for this set of parameters $L=5$ is the optimal choice for the sample-size.} \blue{Final conclusion. Good, except that it is not entirely true. What you know is that $L=2$ is too little and that $L=10$ is too much. The optimum is in between but you don't really know.}

{The stochastic gradients $\hbs(\bbw,\tbtheta)$ in \eqref{stochastic_gradient} are computed as an average of $L$ sample gradients $\nabla f(\bbw,{\bbtheta_{l}})$. To study the effect of the choice of $L$ on RES we consider problems as in \eqref{example_problem} with matrices $\bbA$ and vectors $\bbb$ generated as in Section \ref{sec_numerical_analysis_condition_number}.} {We consider problems with $n=50$, $\theta_0=0.5$, and $\xi=2$; set the RES parameters to $\delta=10^{-3}$ and $\Gamma=10^{-4}$; and the step size sequence to $\epsilon_{t}=\epsilon_{0}T_{0} / (T_{0}+t)$ with  $\epsilon_{0} =10^{-1}$ and $T_{0}=10^3$. We then consider different choices of $L$ and for each specific value generate {$J=1,000$} problem instances. For each run we record the total number $\tau_L$ of sample functions that need to be processed to achieve relative distance to optimality $\|\bbw_t-\bbw^*\|/\|\bbw^*\| \leq10^{-2}$ [cf. \eqref{eqn_empirical_convergence_time}].  If $\tau>10^4$ we report $\tau=10^4$ and interpret this outcome as a convergence failure. The resulting estimates of the probability distributions of the times $\tau_L$ are reported in Fig. \ref{fig:SSE} for $L=1$, $L=2$, $L=5$, $L=10$, and $L=20$.} 

{The trends in convergence times $\tau$ apparent in Fig. \ref{fig:SSE} are: (i) As we increase $L$ the variance of convergence times decreases. (ii) The average convergence time decreases as we go from small to moderate values of $L$ and starts increasing as we go from moderate to large values of $L$.}
 {Indeed, the empirical standard deviations of convergence times decrease monotonically from $\sigma_{\tau_1} = 2.8 \times 10^{3}$ to $\sigma_{\tau_2} = 2.6 \times 10^{2}$, $\sigma_{\tau_5} = 31.7$, $\sigma_{\tau_{10}} = 28.8$, and $\sigma_{\tau_{20}} = 22.7$, when $L$ increases from $L=1$ to $L=2$, $L=5$, $L=10$, and $L=20$. The empirical mean decreases from $\bar\tau_{1} =3.5 \times 10^{3} $ to $\bar\tau_{2} = 6.3 \times 10^{2}$ as we move from $L=1$ to $L=2$, stays at about the same value $\bar\tau_{5} = 3.3 \times 10^{2}$ for $L=5$ and then increases to $\bar\tau_{10} = 5.8 \times 10^{2} $ and $\bar\tau_{20} =1.2 \times 10^{3} $ for $L=10$ and $L=20$.} {This behavior is expected since increasing $L$ results in curvature estimates $\hbB_t$ closer to the Hessian $\bbH(\bbw_t)$ thereby yielding better convergence times. As we keep increasing $L$, there is no payoff in terms of better curvature estimates and we just pay a penalty in terms of more function evaluations for an equally good $\hbB_t$ matrix. This can be corroborated by observing that the convergence times $\tau_{5}$ are about half those of $\tau_{10}$ which in turn are about half those of $\tau_{20}$. This means that the {\it actual} convergence times $\tau/L$ have similar distributions for $L=5$, $L=10$, and $L=20$.} {The empirical distributions in Fig. \ref{fig:SSE} show that moderate values of $L$ suffice to provide workable curvature approximations. This justifies the use $L=5$ in sections \ref{sec_numerical_analysis_condition_number} and \ref{sec_numerical_analysis_problem_dimension}}
 
%\red{Further observe that proper selection of $L$ is important to improve convergence times but irrespectively of the particular choice RES outperforms SGD. To see that this is true just observe that the parameters in this section are as in Fig. \ref{fig:2} where we can see that for SGD the median of sample gradient evaluations to achieve convergence is $\text{median}{(\tau')=7.3 \times10^3}$ sample gradient evaluations to achieve convergence. This is more than the worst RES case that the median of required sample gradient is $\text{median}{(\tau_{1})=2.6 \times10^3}$.} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

\begin{figure*}[t]
        \centering
        \begin{subfigure}[b]{0.5\textwidth}
                \includegraphics[width=\textwidth]{n=5.eps}
                \caption{$n = 5$}
                \label{fig:n=5}
        \end{subfigure}%
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad etc.
          %(or a blank line to force the subfigure onto a new line)
        \begin{subfigure}[b]{0.5\textwidth}
                \includegraphics[width=\textwidth]{n=10.eps}
                \caption{$n=10$}
                \label{fig:n=10}
        \end{subfigure}
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad etc.
          %(or a blank line to force the subfigure onto a new line)
        \begin{subfigure}[b]{0.5\textwidth}
                \includegraphics[width=\textwidth]{n=20.eps}
                \caption{$n=20$}
                \label{fig:n=20}
        \end{subfigure}%
           ~ %add desired spacing between images, e. g. ~, \quad, \qquad etc.
          %(or a blank line to force the subfigure onto a new line)
        \begin{subfigure}[b]{0.5\textwidth}
                \includegraphics[width=\textwidth]{n=50.eps}
                \caption{$n=50$}
                \label{fig:n=50}
        \end{subfigure}
        \caption{ Histogram of the number of data points that SGD and RES needs to converge. Convergence time for RES increases smoothly by increasing the dimension of problem, while convergence time of SGD increases faster.  }\label{fig:dimension}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsection{Effect of problem's dimension}\label{sec_numerical_analysis_problem_dimension}

To evaluate performance for problems of different dimensions we consider functions of the form in \eqref{example_problem} with $\bbb$ uniformly chosen from the box $[0,1]^n$ and diagonal matrix $\bbA$ as in Section \ref{sec_numerical_analysis_condition_number}. However, we select the elements $a_{ii}$ as uniformly drawn from the interval $[0,1]$. This results in problems with more moderate condition numbers and allows for a comparative study of performance degradations of RES and SGD as the problem dimension $n$ grows. 

{The variability parameter for the random vector $\bbtheta$ is set to $\theta_0=0.5$. The RES parameters are $L=5$, $\delta=10^{-3}$, and $\Gamma=10^{-4}$. For SGD we use $L=1$. In both methods the step size sequence is $\epsilon_{t}=\epsilon_{0}T_{0} / (T_{0}+t)$ with  $\epsilon_{0} =10^{-1}$ and $T_{0}=10^3$. For a problem of dimension $n$ we study convergence times $\tau_n$ and $\tau'_n$ of RES and SGD as defined in \eqref{eqn_empirical_convergence_time} with $\rho=1$. For each value of $n$ considered we determine empirical distributions of $\tau_n$ and $\tau'_n$ across $J=1,000$ problem instances. If $\tau>5 \times 10^5$ we report $\tau= 5 \times 10^5$ and interpret this outcome as a convergence failure. The resulting histograms are shown in Fig. \ref{fig:dimension} for $n=5$, $n=10$, $n=20$, and $n=50$.} 

%\red{In Fig. \ref{fig:n=5} where the dimension of problem is $n=5$,  the mean for the number of data points that regularized stochastic BFGS needs to converge is $383$ while the mean for SGD is $975$, but the median for regularized stochastic BFGS is $400$ and for SGD is $265$. The reason is that for SGD when the condition number is very large more than $10^5$ points is needed for convergence. Since the dimension is not very large it does not happen often and the probability is small for this event. This mass increases the mean, but can not change the median. On the other hand, regularized stochastic BFGS is very consistent and the median and mean are very close and the variance is  $3.78\times10^{3}$ for BFGS while the variance for SGD is $2.51\times10^{8}$.} \blue{This was very good. The only problem is that the isntance at $10^5$ screws up your numbers. I rewrote this obviating the mean and standard deviation and writing only about the median and some interval spread characterizations.}
 {For problems of small dimension having $n=5$ the average performances of RES and SGD are comparable, with SGD performing slightly better. E.g., the medians of these times are $\text{median}(\tau_5)=400$ and $\text{median}(\tau'_5)=265$, respectively. A more significant difference is that times $\tau_5$ of RES are more concentrated than times $\tau'_5$ of SGD. The latter exhibits large convergence times $\tau'_5>10^3$ with probability {$0.06$} and fails to converge altogether in a few rare instances -- we have $\tau'_5=5\times10^5$ in {1 out of 1,000 realizations}. In the case of RES all realizations of $\tau_5$ are in the interval {$70\leq\tau_5\leq1095$}}. 

As we increase $n$ we see that RES retains the smaller spread advantage while eventually exhibiting better average performance as well. Medians for $n=10$ are still comparable at {$\text{median}(\tau_{10})=575$ and $\text{median}(\tau'_{10})=582$}, as well as for $n=20$ at {$\text{median}(\tau_{20})=745$ and $\text{median}(\tau'_{20})=1427$}. For $n=50$ the RES median is decidedly better since {$\text{median}(\tau_{50})=950$ and $\text{median}(\tau'_{50})=7942$}. 

For large dimensional problems having $n=50$ SGD becomes unworkable. It fails to achieve convergence in $5 \times 10^5$ iterations with probability $0.07$ and exceeds $10^4$ iterations {with probability $0.45$}. For RES we fail to achieve convergence in $5\times 10^5$ iterations with probability $3\times10^{-3}$ and achieve convergence in less than $10^4$ iterations in all other cases. Further observe that RES degrades smoothly as $n$ increases. The median number of gradient evaluations needed to achieve convergence increases by a factor of {$\text{median}(\tau'_{50})/\text{median}(\tau'_{5}) = 29.9$} as we increase $n$ by a factor of $10$. The spread in convergence times remains stable as $n$ grows.

%\red{Fig. \ref{fig:n=50} studies the case that $n=50$. there is a big probability $0.07$ that SGD needs more than $5\times10^{5}$ data points to converge. For regularized stochastic BFGS also there is a positive probability to converge with more than $5\times10^{5}$, but the probability is $3\times10^{-3}$ which is very small and it belong sot the case that the condition number is more than $10^{6}$. As Fig. \ref{fig:n=50} shows with probability $0.997$ the number of necessary data points for convergence is less than $3515$ in regularized stochastic BFGS. The mean, median and variance for SGD are $5.89\times10^{4}$, $7942$ and $1.77\times 10^{10}$, respectively,  while these number for regularized stochastic BFGS are $2.86\times10^{3}$, $950$ and $9.75\times10^8$.} \blue{Remove this paragraph. I left it here because there are useful numbers that I didn't have time to copy onto earlier paragraphs.}



==> bibi.tex <==
\begin{thebibliography}{6}

\bibitem{Ribeiro10}
A.~Ribeiro, \emph{Ergodic stochastic optimization algorithms for wireless communication and networking}, .\hskip 1em plus
  0.5em minus 0.4em\relax IEEE Trans. Signal Process., vol. 58, no. 12, pp. 6369-6386, December 2010.
\\    
\bibitem{Ribeiro12}
A.~Ribeiro, \emph{Optimal resource allocation in wireless communication and networking}, .\hskip 1em plus
 0.5em minus 0.4em\relax EURASIP J. Wireless commun., vol. 2012, no. 272, August 2012.
\\    
\bibitem{Broyden}
C.~G.~Broyden,~J.~E.~Dennis~Jr. and ~J.~J.~More, \emph{On the local and superlinear convergence of quasi-Newton methods}, .\hskip 1em plus
 0.5em minus 0.4em\relax IMA J. Appl. Math, vol. 12, Issue 3, pp. 223-245, 1973.    
\\    
\bibitem{Byrd}
R.~H.~Byrd,~J.~Nocedal and~Y.~Yuan, \emph{Global convergence of a class of quasi-Newton methods on convex problems}, .\hskip 1em plus
 0.5em minus 0.4em\relax SIAM J. Numer. Anal., vol. 24, Issue 5, pp. 1171-1190, October 1987.     
 \\
 \bibitem{Nocedal}
J.~Nocedal and S.~J.~Wright, \emph{Numerical optimization}, 2nd~ed.\hskip 1em plus
  0.5em minus 0.4em\relax Springer Series in Operations Research. Springer-Verlag, New York, NY., 1999.    
  \\
  \bibitem{Powell}
Powell,~M.~J.~D., \emph{Some properties of the variable metric method}, 2nd~ed.\hskip 1em plus
  0.5em minus 0.4em\relax In numerical methods for non-linear optimization, London: Academic Press, 1972.     
\\
\bibitem{Boyd}
S.~Boyd and L.~Vandenberghe, \emph{Convex Optimization}, \hskip 1em plus
  0.5em minus 0.4em\relax Cambridge, U.K.: Cambridge Univ. Press, 2004.    
\\
\bibitem{Solo}
V.~Solo and X.~Kong, \emph{Adaptive Signal Processing Algorithms: Stability
and Performance} \hskip 1em plus
  0.5em minus 0.4em\relax Englewood Cliffs, NJ: Prentice-Hall, 1995.
  
\end{thebibliography}
